ShotVL: Human-Centric Highlight Frame Retrieval via Language Queries

Existing works on human-centric video understanding typically focus on analyzing specific moment or entire videos. However, many applications require higher precision at the frame level. In this work, we propose a novel task, BestShot, which aims to locate highlight frames within human-centric videos via language queries. This task demands not only a deep semantic comprehension of human actions but also precise temporal localization. To support this task, we introduce the BestShot Benchmark. %The benchmark is meticulously constructed by combining human detection and tracking, potential frame selection based on human judgment, and detailed textual descriptions crafted by human input to ensure precision. The benchmark is meticulously constructed by combining human-annotated highlight frames, detailed textual descriptions and duration labeling. These descriptions encompass three critical elements: (1) Visual content; (2) Fine-grained action; and (3) Human Pose Description. Together, these elements provide the necessary precision to identify the exact highlight frames in videos. To tackle this problem, we have collected two distinct datasets: (i) ShotGPT4o Dataset, which is algorithmically generated by GPT-4o and (ii) Image-SMPLText Dataset, a dataset with large-scale and accurate per-frame pose description leveraging PoseScript and existing pose estimation datasets. Based on these datasets, we present a strong baseline model, ShotVL, fine-tuned from InternVL, specifically for BestShot. We highlight the impressive zero-shot capabilities of our model and offer comparative analyses with existing SOTA models. ShotVL demonstrates a significant 52% improvement over InternVL on the BestShot Benchmark and a notable 57% improvement on the THUMOS14 Benchmark, all while maintaining the SOTA performance in general image classification and retrieval.

==> abs.tex <==
\begin{abstract}
%This study introduces the \textbf{BestShot} task, which focuses on capturing highlight frames in videos through language queries. 
%Although methods initially designed for tasks like Image Aesthetic Assessment, Temporal Action Localization, and Moment Retrieval can be adapted to identify highlight frames in videos, they have certain limitations, such as focusing solely on image aesthetics, covering limited action categories, or only retrieving time segments.  
%Considering the limitations of existing benchmarks, we propose a novel frame-retrieval-in-videos benchmark for evaluating the BestShot task, called \textbf{BestShot Benchmark}. It comprises 4,500 manually crafted queries of highlight frames extracted from over 1,000 sequences sampled from THUMOS14 and FineAction. 
%Although Contrastive Language-Image Pre-training (CLIP) and subsequent models based on its architecture have demonstrated effectiveness on the BestShot task, they still struggle with distinguishing subtle differences in action and pose between adjacent frames, as well as understanding temporal information. 
%To address these issues, we propose: \textbf{(i) ShotGPT4o Dataset}: a dataset generated by GPT4o. This dataset provides frame-level action and pose descriptions, as well as video-level question-answer pairs (QAs) related to frame or moment retrieval. It consists of 200,000 image instruction data and 150,000 video instruction data, covering 1,500 action categories. \textbf{(ii) ImageSMPLText Dataset}: a large-scale dataset based on PoseScript, featuring 18.6 million frame pose descriptions from 69,000 videos and 13 open datasets. \textbf{(iii) ShotCLIP}: A robust baseline for the BestShot task, comprising ShotCLIP-Base and ShotCLIP-Chat. ShotCLIP outperforms InternVL, the state of the art open-source vision-language model, by 52\% on the BestShot Benchmark and by 25\% on THUMOS14 zero-shot temporal action localization. It also surpasses CLIP by 107\% on BestShot and by 63\% on THUMOS14.
%Dataset and code is available at: \href{https://github.com/shotclip/shotclip.github.io/}{https://github.com/shotclip/shotclip.github.io} 


%\color{blue}Multimodal Pre-trained Models have demonstrated effectiveness on various vision tasks. However, these models are predominantly designed for generalizability, focusing on the overall video rather than abundant frames. This limitation hinders the ability of existing models to accurately locate specific frames via language queries. The absence of precise task definition and standard benchmarks further exacerbates this challenge. To address this issue, we first introduce the \textbf{BestShot} task and a novel frame-retrieval-in-videos benchmark, \textbf{BestShot Benchmark}. Unlike traditional tasks, BestShot is specifically designed capturing highlight frames in videos through language queries. Furthermore, we also propose \textbf{ShotCLIP}, a robust baseline for this task, augmented with two datasets: \textbf{(i) ShotGPT4o Dataset}, a dataset generated by GPT4o and \textbf{(ii) ImageSMPLText Dataset}, a large-scale dataset based on PoseScript. ShotCLIP outperforms InternVL, the state of the art open-source vision-language model, by 52\% on the BestShot Benchmark and by 25\% on THUMOS14 zero-shot temporal action localization. It also surpasses CLIP by 107\% on BestShot and by 63\% on THUMOS14.

This study introduces the \textbf{BestShot} task, which aims to locate highlight frames in videos through language queries. 
While existing methods initially designed for tasks like Image Aesthetic Assessment, Temporal Action Localization, and Moment Retrieval can be adapted to identify highlight frames in videos, they exhibit certain limitations, such as focusing solely on image aesthetics, covering limited action categories, or retrieving only time segments. 
To better address these challenges, we first propose the task \textbf{BestShot} alongside with an associated benchmark, named \textbf{BestShot Benchmark}. This benchmark is designed to assess a model's ability to localize an exact frame in human-centric videos using language queries.
Furthermore, we claim the following contributions: 
\textbf{(i) Pre-Summary Sliding-Shot (PreS3) Captioning Strategy}: A video captioning strategy utilizing GPT4o to generate accurate question-answer pairs (QAs) related to frame retrieval, moment retrieval, and other general video comprehension tasks. Applying this strategy, We present the ShotGPT4o dataset that includes frame-level descriptions and QAs.
%\textbf{(i) ShotGPT4o Dataset}: A dataset generated using the Pre-Summary Sliding-Shot(PreS3)} Captioning Strategy. It uses GPT4o to generate accurate question-answer pairs (QAs) related to frame retrieval, moment retrieval and other general video QAs.
\textbf{(ii) ImageSMPLText Dataset}: A large-scale dataset derived from PoseScript, featuring millions of fine-grained pose descriptions paired with real-world video frames. 
\textbf{(iii) ShotVL}: A robust baseline finetuned from InternVL for the BestShot task, comprising ShotVL-Base and ShotVL-Chat. 
We highlight the powerful zero-shot capability of our model and provide comparisons with state-of-the-art models. 
ShotCLIP achieves a 56\% improvement over InternVL on the BestShot Benchmark and a 25\% improvement on THUMOS14. 
Additionally, our model preserves the general image classification and retrieval abilities from the pre-trained model, contrasting with conventional fine-tuning models.
\end{abstract}
